Opportunistic Decoding with Timely Correction for Simultaneous Translation

Simultaneous translation has many important application scenarios and attracts much attention from both academia and industry recently. Most existing frameworks, however, have difficulties in balancing between the translation quality and latency, i.e., the decoding policy is usually either too aggressive or too conservative. We propose an opportunistic decoding technique with timely correction ability, which always (over-)generates a certain mount of extra words at each step to keep the audience on track with the latest information. At the same time, it also corrects, in a timely fashion, the mistakes in the former overgenerated words when observing more source context to ensure high translation quality. Experiments show our technique achieves substantial reduction in latency and up to +3.1 increase in BLEU, with revision rate under 8% in Chinese-to-English and English-to-Chinese translation.

==> Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

#SHELL = /bin/sh
#MAKE  = gmake

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmode
TEX = latex 

######################################################################
# source files

texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib *.bst)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty *.cls)

figfiles  = $(wildcard figures/*.fig)
figfiles += $(wildcard figures/*.plt)
figfiles += $(wildcard diagram-*.pdf)
figfiles += $(wildcard figures/*.tex)
figfiles += $(wildcard figures/*.ps)
figfiles += $(wildcard figures/*.epsi)
figfiles += $(wildcard figures/*.c)
figfiles += $(wildcard figs/*.eps)
figfiles += $(wildcard figs/*.gnuplot)
figfiles += $(wildcard figs/*.mp)
figfiles += $(wildcard figs/*.pdf)
figfiles += $(wildcard figs/*.tex)


figfiles += $(wildcard figures/apps/*.fig)
figfiles += $(wildcard figures/apps/*.plt)
figfiles += $(wildcard figures/apps/*.pdf)
figfiles += $(wildcard figures/apps/*.ps)
figfiles += $(wildcard figures/apps/*.epsi)
figfiles += $(wildcard figures/apps/*.c)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.bbl)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)
#tmp_files += (texput.log)

######################################################################
# output files

target =main

######################################################################
# make targets

all:  pdf

simple:
	latex ${target}; dvips -t letter ${target}.dvi -o ${target}.ps


dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
#	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	@${TEX} $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -t letter -P pdf -G0 -q -o $@ $<

#%.pdf : %.ps
#	ps2pdf $< $@
#	~/local/macscripts/refresh.scpt

#	cd figs; mptopdf *.mp; cd ..

# %.pdf: %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
# 	pdflatex ${*F} #> ${*F}.log
# 	#tail ${*F}.log
# 	@if  grep Citation ${*F}.log ; then \
# 		bibtex ${*F};   \
# 		pdflatex ${*F};      \
# 		bibtex ${*F};   \
# 		pdflatex ${*F}
# 	#fi
# 	#open $@
# #	~/local/macscripts/refresh.scpt

fast:
	pdflatex main

%.pdf : %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
#	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	#pdflatex si
	pdflatex $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		pdflatex $<;	\
		pdflatex $<;	\
	fi
	#@-/bin/rm -f ${tmp_files}
	#pdfcrop --margin "5 5 5 5" main.pdf
	# open main-crop.pdf
	gs -sDEVICE=pdfwrite -dNOPAUSE -dBATCH -dSAFER \
       -dFirstPage=1 -dLastPage=5 \
       -sOutputFile=paper.pdf main.pdf
	gs -sDEVICE=pdfwrite -dNOPAUSE -dBATCH -dSAFER \
       -dFirstPage=6 \
       -sOutputFile=appendix.pdf main.pdf


long.bib:	all.bib
	./remove-short.pl all.bib > long.bib


######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile

paper.pdf:	${target}.pdf
	gs -q -sPAPERSIZE=letter -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -dFirstPage=1 -dLastPage=12 main.pdf

si.pdf:	${target}.pdf
	gs -q -sPAPERSIZE=letter -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -dFirstPage=13 -dLastPage=20 main.pdf




==> defs_emnlp.tex <==
% !TEX root = main.tex

\newcommand{\state}{(\vecs, \vect)\xspace}
\newcommand{\seq}{(\vecx, \vecy)\xspace}
\newcommand{\vecP}{\ensuremath{\mathbf{P}}\xspace}

\newcommand{\delay}{\langle \varepsilon \rangle\xspace}
\newcommand{\pixyofst}{\pi^\star_{\vecx, \vecy} ((\vecs, \vect))\xspace}
\newcommand{\pixy}{\pi^\star_{\vecx, \vecy}\xspace}
\newcommand{\pixyabofst}{\pi^\star_{\vecx, \vecy, \alpha, \beta} ((\vecs, \vect))\xspace}
\newcommand{\pixyab}{\pi^\star_{\vecx, \vecy, \alpha, \beta}\xspace}
\newcommand{\piofs}{\pi^\star_{\vecx, \vecy, \alpha, \beta}(s)\xspace}
\newcommand{\piofsi}{\pi^\star_{\vecx, \vecy, \alpha, \beta}(s_i)\xspace}

\newcommand{\tuple}[1]{\ensuremath{\langle {#1} \rangle}}
%\newcommand{\argmax}[2]{\ensuremath{\mbox{argmax}_{#1}\ {#2}}}

\newcommand{\featuresum}[1]{\ensuremath{\sum_i \lambda_i f_i({#1})}}

\newcommand{\fvec}[1]{\ensuremath{\vec{f} ({#1})}}

\newcommand{\fiof}[1]{\ensuremath{f_i ({#1})}}

\newcommand{\fofi}[0]{\ensuremath{f_i}}

\newcommand{\featureprod}[1]
{\ensuremath{\vec{\lambda} \cdot \fvec{#1} } }

\newcommand{\efprod}[1]{\ensuremath{e^{\featureprod{#1}}}}
\newcommand{\efsum} [1]{\ensuremath{e^{\featuresum {#1}}}}

\newcommand{\lami}{\ensuremath{\lambda_i}}

\newcommand{\empExp}[1]{\ensuremath{\mbox{\~{E}} [{#1}]}}
\newcommand{\expect}{\ensuremath{\mathbb{E}}}

\newcommand{\ks}{\ensuremath{k}}
\newcommand{\Ks}{\ensuremath{K}}
\newcommand{\kbest}{\ks-best\xspace}
\newcommand{\topk}{top-\ks\xspace}
\newcommand{\kBest}{\Ks-Best\xspace}

\newcommand{\notes}[1]{}%{\it {\small {#1}}}}

\newcommand{\acite}[1]{({--#1})}

\newcommand{\define}[1]{{\bf Definition.} {\em {#1}}}
\newcommand{\zerobar}{\ensuremath{\overline{0}}\xspace}
\newcommand{\onebar}{\ensuremath{\overline{1}}\xspace}

\newcommand{\Items}{\ensuremath{\mathcal{I}}\xspace}

\newcommand{\oplusk}{\ensuremath{\oplus_{\tiny k}}}
\newcommand{\otimesk}{\ensuremath{\otimes_{\tiny k}}}

\newcommand{\zerok}{\ensuremath{\overline{0}^k}\xspace}
\newcommand{\onek}{\ensuremath{\overline{1}^k}\xspace}

\newcommand{\scalar}{\ensuremath{\odot_k}}

\newcommand{\kdim}{\ks-dimensional\ }





% \newlistof{defin}{def}{List of Definitions}

% \newcommand{\defin}[1]{%
% \refstepcounter{defin}
% \par\noindent\textbf{Definition \thedefin. #1}
% \addcontentsline{ans}{defin}{\protect\numberline{\thedefin}#1}\par}

% for amsthm
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{definition}[theorem]{Definition}

\newcommand{\gc}{\ensuremath{|G|}\xspace}
\newcommand{\ntsize}{\ensuremath{|N|}\xspace}
\newcommand{\nt}{\ensuremath{N}\xspace}
\newcommand{\rulepernt}{\ensuremath{R}\xspace}

\newcommand{\Ttimesk}{\ensuremath{T_{\otimesk}}\xspace}
\newcommand{\Tplusk}{\ensuremath{T_{\oplusk}}\xspace}
\newcommand{\maxk}{\ensuremath{\mbox{\bf max}_k}\xspace}

\newcommand{\tenexp}[1]{\ensuremath{10^{{-#1}}}\xspace}

\newcommand{\naive}{na\"{\i}ve\xspace}

\newcommand{\perc}[1]{\ensuremath{{#1}\%}\xspace}

\newcommand{\veca}{\ensuremath{\mathbf{a}}\xspace}
\newcommand{\vecb}{\ensuremath{\mathbf{b}}}
\newcommand{\vecp}{\ensuremath{\mathbf{p}}}
\newcommand{\klogk}{\ensuremath{k\log k}}
\newcommand{\vecz}{\ensuremath{\mathbf{z}}}
\newcommand{\vech}{\ensuremath{\bm{h}}}
\newcommand{\vecW}{\ensuremath{\mathbf{W}}}
\newcommand{\vecs}{\ensuremath{\mathbf{s}}\xspace}
\newcommand{\vect}{\ensuremath{\mathbf{t}}\xspace}
\newcommand{\better}{\ensuremath{\preceq}}


\newcommand{\opt}{\ensuremath{\mbox{{\bf min}}_\better}}
\newcommand{\mergek}{\ensuremath{\mbox{{\bf merge}}_{\better k}}\xspace}
\newcommand{\multk}{\ensuremath{\mbox{{\bf mult}}_{\better k}}\xspace}

\newcommand{\kw}{\ensuremath{\mathbf{w}}}

\newcommand{\kwi}{\ensuremath{w_i}}
\newcommand{\wejv}[3]{\ensuremath{w^{#1}_{{#2}}({#3})}}

\newcommand{\vecj}{\ensuremath{\mathbf{j}}}
\newcommand{\vecD}{\ensuremath{\mathbf{D}}}
\newcommand{\vecu}{\ensuremath{\mathbf{u}}\xspace}
\newcommand{\vecU}{\ensuremath{\mathbf{U}}}
\newcommand{\vecjhat}{\ensuremath{\hat{\mathbf{j}}}}
\newcommand{\vecone}{\ensuremath{\mathbf{1}}}
\newcommand{\dbp}[2]{\ensuremath{\langle{#1}, {#2}\rangle}}

\newcommand{\reviewtimetoday}[3]{
    \AtBeginDocument{
    \special{
    !userdict begin
    /pagenum 0 def
    /bop-hook
    {
        /pagenum pagenum 1 add def
        pagenum #3 le
        {
        gsave
        430 750 translate
        0 rotate
        0.4 setgray
        /Times-Roman findfont
        10 scalefont setfont
        0 0   moveto
        (#1) show
        0 -10 moveto
        (#2) show
        grestore
        } if
    } def
    }  }}

% for submission
\iffalse
\renewcommand{\marginpar}[1]{}
\fi

%\newcommand{\comment}[1]{\marginpar{\raggedright{\em{\small #1}}}}

\newcommand{\ith}[1]{\ensuremath{i^{{th}}}}
\def\alglazy{Algorithm 3}

\newcommand{\JnM}{Jim\'enez and Marzal\xspace}

%\newcommand{\ind}[1]{\ensuremath{^{(#1)}}}
\newcommand{\srule}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\goesto}{\ensuremath{\rightarrow}\xspace}
\newcommand{\chn}[1]{\mbox{{\it {#1}}}}

\newcommand{\ngram}{\ensuremath{\text{$n$-gram}}\xspace}
\newcommand{\ngrams}{\ensuremath{\text{$n$-grams}}\xspace}

\newcommand{\ngramitem}[5]{
\ensuremath{
\left(
\begin{smallmatrix}
\mbox{\small {#4}} &\cdots & \mbox{\small {#5}} \\
&
%\!\!_{#2}
\mbox{#1}
%_{#3}
 &
\\ {#2} & & {#3}
\end{smallmatrix}
 \right)
}}

\newcommand{\specialngramitem}[7]{
\begin{math}
\left(
\begin{smallmatrix}
\mbox{\small {#2}}\ \cdots\ \mbox{\small{#3}}
& \cdots &
\mbox{\small {#4}}\ \cdots\ \mbox{\small {#5}} \\
& \mbox{{#1}} & \\
{#6} & & {#7}
\end{smallmatrix}
 \right)
\end{math}
}

\newcommand{\chartitem}[3]{
\ensuremath{(\mbox{#1},{#2},{#3})}
}

\newcommand{\vtnt}[1]{\ensuremath{V_{\mbox{\tiny #1}}}}
%%% \bigram{a}{b} means (a,b) is a bigram pair. P (b | a)!
\newcommand{\bigram}[2]{\ensuremath{\Pr(\mbox{\small #2} \mid \mbox{\small #1})}}

\newcount\permx
\newcount\permy
\def\permdot#1#2{
\permx=#1 \advance\permx by-1
\permy=#2 \advance\permy by-1
\psframe[fillcolor=black, fillstyle=solid]
(\permx,\permy)(#1, #2)
}

%%% note: realcalc.sty has a fatal bug : 23-0.5=23.5.
%%% so i have to do this... +1-0.5 thing
\newcommand{\minushalf}[1]{
    \Radd{\aaa}{#1}{-1}
    \Radd{\aaa}{\aaa}{0.5}
    \Rtrunc{\aaa}{1}{\aaa}
    \aaa
}


\newcommand{\permnt}[3]{
\rput({#1},{#2}){\huge\color{white} {#3}}
}


\newcommand\union{\cup}
\newcommand\intersect{\cap}

\newcommand\vecd[2]{\ensuremath{d_{#2}{(#1)}}}
\newcommand\veczero{\ensuremath{\mathbf{0}}}
\newcommand\vecq{\ensuremath{\mathbf{q}}}
\newcommand\vecn{\ensuremath{\mathbf{n}}}
%\newcommand\vecone{\ensuremath{\mathbf{1}}}
\newcommand{\argmax}{\operatornamewithlimits{\mathbf{argmax}}}
\newcommand{\argtop}{\operatornamewithlimits{\mathbf{argtop}}}
\newcommand{\toptop}{\operatornamewithlimits{\mathrm{top}}}
\newcommand{\nextfunc}{\operatornamewithlimits{\mathrm{next}}}
\newcommand{\argmin}{\operatornamewithlimits{\mathbf{argmin}}}

\newcommand{\deltahat}{\ensuremath{\hat{\delta}}\xspace}

\newcommand{\xrs}{{\bf xRs}\xspace}
\newcommand{\xrsln}{\mbox{1-{\bf xRLNs}}\xspace}
\newcommand{\RLN}{{\bf RLN}\xspace}

\newcommand{\x}[1]{\ensuremath{x_{#1}}\xspace}
\newcommand{\foot}[1]{\ensuremath{^{\tiny({#1})}_{\downarrow}}}


\newcommand{\chnprd}{{\tiny \ensuremath{_{\circ}}}}

%\newcommand{\ckyitem}[3]{\ensuremath{(_{#2}{\mbox{#1}}_{#3})}\xspace}
%\newcommand{\ckyitem}[3]{\ensuremath{({\mbox{#1}}_{#2, #3})}\xspace}
\newcommand{\ckyitem}[3]{\ensuremath{{\mbox{#1}}_{{{#2},\,{#3}}}}\xspace}
\newcommand{\treeitem}[2]{\ensuremath{{\mbox{#1}}_{#2}}\xspace}
\newcommand{\nodent}[3]{\ensuremath{\treeitem{#1}{#2}:{#3}}}

\newcommand{\coverage}[1]{\ensuremath{(\mbox{{#1}})}\xspace}
\newcommand{\lmcov}[2]{\ensuremath{(\mbox{#1}, ^{\mbox{\scriptsize #2}}\!)}\xspace}
\newcommand{\phritem}[3]{\ensuremath{\coverage{#1}:({#2}, \mbox{\footnotesize ``#3''})}\xspace}
\newcommand{\lmphritem}[4]{\ensuremath{\lmcov{#1}{#2}:({#3}, \mbox{\footnotesize ``#4''})}\xspace}
\newcommand{\phrpair}[2]{\ensuremath{\langle \mbox{\chn{#1}, {#2}}\rangle}\xspace}

\newcommand{\lmitem}[3]{\ensuremath{({{#1}}^{#2 \star #3})}\xspace}
%\newcommand{\lmckyitem}[5]{\resizebox{!}{.15in}{\ensuremath{(\mbox{\small #1}_{\mbox{\tiny\ {#2},{#3}}}^{\tiny\ \mbox{#4}\ \star\ \mbox{#5}})}}\xspace}
\newcommand{\lmckyitem}[5]{\ensuremath{(\mbox{#1}_{\mbox{\scriptsize\ ({#2},{#3})}}^{\scriptsize\ \mbox{#4}\ \star\ \mbox{#5}})}\xspace}

\def\wlm{$\mathord+\textrm{LM}$\xspace}
\def\wolm{$\mathord-\textrm{LM}$\xspace}

\newcommand{\sym}[1]{\textrm{#1}\xspace}
\newcommand{\VP}{\sym{VP}}
\newcommand{\PP}{\sym{PP}}

\newcommand{\startsym}{\mbox{\scriptsize \texttt{<s>}}\xspace}
\newcommand{\stopsym}{\mbox{\scriptsize \texttt{</s>}}\xspace}
\newcommand{\TOP}{\sym{TOP}}
%\newcommand{\plm}[2]{\ensuremath{P_{lm}(\mbox{\small #2}\mid\mbox{\small #1})}}
\newcommand{\plm}[2]{\ensuremath{P_{lm}(\mbox{#2}\mid\mbox{#1})}}

%\newcommand{\order}[1]{\ensuremath{\mathcal{O}(#1)}}
\newcommand{\order}{\ensuremath{\mathcal{O}}}

\newcommand{\wocombo}{\ensuremath{h}\xspace}
\newcommand{\mincombo}{\ensuremath{h_{\mathit{combo}}}\xspace}

% \renewcommand{\min}{\ensuremath{\mbox{\bf min}}\xspace}
\newcommand{\hyp}[1]{\mbox{\tiny ``{#1}''}}
\newcommand{\hl}{\ensuremath{k}\xspace}


\newcommand{\cand}{\ensuremath{\mathit{cand}}\xspace}
\newcommand{\buf}{\ensuremath{\mathit{buf}}\xspace}
\newcommand{\bound}{\ensuremath{\mathit{bound}}\xspace}

\newcommand{\lazyjbest}{\ensuremath{\textproc{LazyJthBest}}\xspace}

\newcommand{\backwardstar}{\ensuremath{\mathit{IN}}\xspace}

\newtheorem{proposition}[theorem]{Proposition}

\newcommand{\ff}{\ensuremath{\mathbf{f}}\xspace}
\newcommand{\ee}{\ensuremath{\mathbf{e}}\xspace}
\newcommand{\al}{\ensuremath{\mathbf{a}}\xspace}

\newcommand{\pt}{\ensuremath{p_{\mbox{t}}}}
\newcommand{\pd}{\ensuremath{p_{\mbox{d}}}}


\newcommand{\current}{\color{blue}{\fbox{{\bf C}}}\xspace}
\newcommand{\future}{\color{red}{\fbox{{\bf F}}}\xspace}

\newcommand{\boxnum}[1]{{\setlength{\fboxsep}{1pt}\raisebox{1pt}{\hspace{1pt}\fbox{\tiny #1}\hspace{1pt}}}}
\newcommand{\ind}[1]{\ensuremath{_{\kern-0.5pt\boxnum{#1}}}}
\newcommand{\BS}{\ensuremath{\mathit{IN}}\xspace}
\newcommand{\NTX}{\text{X}}
\newcommand{\NTS}{\text{S}}

\def\FS{\mathit{FS}\xspace}
\def\BS{\mathit{BS}\xspace}
\def\bfR{\mathbf{R}\xspace}

\newcommand{\head}{\ensuremath{\mathit{head}}\xspace}
\newcommand{\tails}{\ensuremath{\mathit{tails}}\xspace}

\newcommand{\Deriv}{\ensuremath{\mathscr{D}}\xspace}
\newcommand{\hhat}{\ensuremath{\hat{h}}\xspace}

\newcommand{\opluseq}{\ensuremath{\ \oplus=}\xspace}

\newcommand{\lianheguo}{\chn{Li\'anh\'egu\'o}\xspace}
\newcommand{\jiandu}{\chn{ji\=and\=u}\xspace}


\newcommand{\chnBushi}{\chn{B\`ush\'i}\xspace}
\newcommand{\chnyu}{\chn{y\v{u}}\xspace}
\newcommand{\chnle}{\chn{le}\xspace}
\newcommand{\chnShalong}{\chn{Sh\=al\'ong}\xspace}
\newcommand{\chnBaoweier}{\chn{B\`aow\=eier}\xspace}
\newcommand{\chnjuxing}{\chn{j\v{u}x\'ing}\xspace}
\newcommand{\chnhuitan}{\chn{hu\`it\'an}\xspace}

\newcommand{\mybullet}{\ensuremath{\bullet\hspace{-0.05mm}}}
\newcommand{\myunderscore}{\ensuremath{\mbox{\Large\_}}}

\newcommand{\nocov}{$_0$\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}
\newcommand{\onecov}{\mybullet$_1$\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}
\newcommand{\halfcov}{\mybullet\myunderscore\myunderscore\mybullet\mybullet\mybullet$_{6}$}
\newcommand{\fullcov}{\mybullet\mybullet\mybullet$_{3}$\mybullet\mybullet\mybullet}

%% \newcommand{\nocov}{\ensuremath{_0\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}\xspace}
%% \newcommand{\onecov}{\ensuremath{\mybullet_1\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}\xspace}
%% \newcommand{\halfcov}{\ensuremath{\mybullet\myunderscore\myunderscore\mybullet\mybullet\mybullet_6}\xspace}
%% \newcommand{\fullcov}{\ensuremath{\mybullet\mybullet\mybullet_3\mybullet\mybullet\mybullet}\xspace}
\newcommand{\fullncov}{\mybullet\mybullet\ldots\mybullet}


\long\def\signature#1{%
% \begin{flushleft}
\begin{center}
% \begin{minipage}{6in}
\parindent=0pt
\shortstack{\vrule width 3in height 0.4pt\\ #1}
% \end{minipage}
\end{center}
% \end{flushleft}
}

% forest rerank acl 2008
\newcommand{\feat}[1]{{\bf {#1}}}
\newcommand{\Gen}[1]{\ensuremath{\mathit{cand}({#1})}\xspace}
\newcommand{\yhat}{\ensuremath{\hat{y}}\xspace}
\newcommand{\ystar}{\ensuremath{y^*}\xspace}
\newcommand{\yplus}{\ensuremath{y^+}\xspace}
\newcommand{\cost}{\ensuremath{\mathit{c}}\xspace}
\newcommand{\oracle}{\ensuremath{\mathit{oracle}}\xspace}
\newcommand{\ora}{\ensuremath{\mathit{ora}}\xspace}
\newcommand{\cnj}{charniak+johnson:2005}
\newcommand{\coll}{collins:2000}
\newcommand{\dom}{\ensuremath{\mathit{dom}}\xspace}
\newcommand{\gold}{\ensuremath{\mathit{gold}}\xspace}

\newcommand{\myoval}[1]{\ovalnode[linestyle=none,fillstyle=solid,fillcolor=lightgray]{foo}{#1}}
\newcommand{\mybox}[1]{\psframebox[linestyle=none,linewidth=0pt,fillstyle=solid,fillcolor=lightgray]{#1}}

\newcommand{\vecx}{\ensuremath{\bm{x}}\xspace}
\newcommand{\vecy}{\ensuremath{\bm{y}}\xspace}
\newcommand{\vecw}{\ensuremath{\mathbf{w}}\xspace}
\newcommand{\vecc}{\ensuremath{\mathbf{c}}\xspace}
\newcommand{\vecR}{\ensuremath{\mathbb{R}}\xspace}

\newcommand{\vecv}{\ensuremath{\mathbf{v}}\xspace}
\newcommand{\vecf}{\ensuremath{\mathbf{f}}\xspace}
\newcommand{\vecfl}{\ensuremath{\mathbf{f}_L}\xspace}
%\newcommand{\veczero}{\ensuremath{\mathbf{j}}}

\newcommand{\heap}{\ensuremath{\mathit{heap}}\xspace}

\newcommand{\feature}[1]{$\langle$ {#1} $\rangle$\xspace}

\newcommand{\defineq}{\ensuremath{\; \triangleq\; }\xspace}
\newcommand{\extradgt}{\color{white}{0}\xspace}

\newcommand{\funit}{\ensuremath{\mathring{f}}\xspace}
\newcommand{\vecfunit}{\ensuremath{\mathring{\vecf}}\xspace}
\newcommand{\Done}[1]{\ensuremath{D_1(#1)}}

% kbest paper 2005
\let\algsize\normalsize
\newcommand{\algline}[2]{%
\begin{center}
\algsize$\text{#1:}\hspace{1em}#2$
\end{center}}

\def\Dhat{\hat{D}}
\def\vecDhat{\mathbf{\hat{D}}}

%%%%%%%%%%%%%%% pinyins

\newcommand{\Baoweier}{\chn{B\`aow\=eier}\xspace}
\newcommand{\Bushi}{\chn{B\`ush\'i}\xspace}
\newcommand{\bushi}{\Bushi}
\newcommand{\Shalong}{\chn{Sh\=al\'ong}\xspace}
\newcommand{\yu}{\chn{y\v{u}}\xspace}
\newcommand{\hai}{\chn{h\'ai}\xspace}
\newcommand{\jiang}{\chn{ji\=ang}\xspace}
\newcommand{\huiwu}{\chn{hu\`iw\`u}\xspace}
\newcommand{\jinyibu}{\chn{j\`iny\={\i}b\`u}\xspace}
\newcommand{\juxing}{\chn{j\v{u}x\'ing}\xspace}
\newcommand{\huitan}{\chn{hu\`it\'an}\xspace}
\newcommand{\dangtian}{\chn{d\=angti\=an}\xspace}
\newcommand{\jiu}{\chn{ji\`u}\xspace}
\newcommand{\zhongdong}{\chn{zh\=ongd\=ong}\xspace}
\newcommand{\weiji}{\chn{w\=eij\=\i}\xspace}
\newcommand{\fuze}{\chn{f\`uz\'e}\xspace}

\newcommand{\zongtong}{\chn{z\v{o}ngt\v{o}ng}\xspace}
\newcommand{\zai}{\chn{z\`ai}\xspace}
\newcommand{\mosike}{\chn{M\`os\-{i}k\={e}}\xspace}
\newcommand{\pujing}{\chn{P\v{u}j\={\i}ng}\xspace}
\newcommand{\eluosi}{\chn{\'Elu\'os\=\i}\xspace}
\newcommand{\meiguo}{\chn{M\v{e}igu\'o}\xspace}
%\dangju & \dui & \shate & \jiezhe & \shizong & \yi & \an &\gandao &  \danyou \\
\newcommand{\dangju}{\chn{d\=angj\'u}\xspace}
\newcommand{\dui}{\chn{du\`\i}\xspace}
\newcommand{\shate}{\chn{Sh\=at\`e}\xspace}
\newcommand{\jiezhe}{\chn{j\`{\i}zh\v{e}}\xspace}
\newcommand{\shizong}{\chn{sh\={\i}z\=ong}\xspace}
\newcommand{\danyou}{\chn{d\=any\=ou}\xspace}
\newcommand{\gandao}{\chn{g\v{a}nd\`ao}\xspace}
\newcommand{\an}{\chn{\`an}\xspace}
\newcommand{\yi}{\chn{y\=\i}\xspace}
\newcommand{\buman}{\chn{b\`um\v{a}n}\xspace}

\newcommand{\Prob}{\ensuremath{\mathrm{P}}\xspace}

\newcommand{\lhs}{\ensuremath{\mathit{lhs}}\xspace}
\newcommand{\rhs}{\ensuremath{\mathit{rhs}}\xspace}

\newcommand{\NULL}{\ensuremath{\mathit{null}}\xspace}

\newcommand{\gap}{\ensuremath{\sqcup}\xspace}
\newcommand{\spanof}{\ensuremath{\mathit{span}}\xspace}
\newcommand{\yield}{\ensuremath{\mathit{yield}}\xspace}
\newcommand{\fs}{\ensuremath{\mathit{admset}}\xspace}

\newcommand{\closed}{\ensuremath{\mathit{closed}}\xspace}
\newcommand{\open}{\ensuremath{\mathit{open}}\xspace}
\newcommand{\hs}{\frag} %\ensuremath{\mathit{frag}}\xspace}
\newcommand{\vs}{\ensuremath{\mathit{vs}}\xspace}
\newcommand{\frag}{\ensuremath{\mathit{frag}}\xspace}
\renewcommand{\root}{\ensuremath{\mathit{root}}\xspace}
\newcommand{\leaves}{\yield} %\ensuremath{\mathit{leaves}}\xspace}
\newcommand{\exps}{\ensuremath{\mathit{front}}\xspace} % frontier
\newcommand{\newexps}{\ensuremath{\mathit{\exps'}}\xspace}


\newcommand{\PLM}{\ensuremath{\Prob_{\mathrm{lm}}}\xspace}
\newcommand{\PT}{\ensuremath{\Prob}\xspace}
\newcommand{\PLex}{\ensuremath{\Prob_{\mathrm{lex}}}\xspace}

\newcommand{\GHKM}[3]{\ensuremath{{\mbox{#1}}_{{#2}}^{{#3}}}\xspace}
%\newcommand{\newGHKM}[2]{\ensuremath{{\mbox{#1}}\\{\mbox{\scriptsize #2}}}\xspace}
\newcommand{\tspan}[1]{\scriptsize {#1}\xspace}
\newcommand{\wnode}[1]{\rnode[t]{#1}{#1}\xspace}  %% target words

\newcommand{\vtitem}[2]{\ensuremath{({\vtnt{#1}}_{#2})}\xspace}
%\newcommand{\gap}{\ensuremath{\sqcup}}
%\newcommand{\treeitem}[2]{\ensuremath{({\mbox{#1}}_{#2})}\xspace}

\newcommand{\ruleset}{\ensuremath{\mathcal{R}}\xspace}

% pattern-match
\newcommand{\match}{\ensuremath{\mathit{match}}\xspace}
\newcommand{\vars}{\ensuremath{\mathit{vars}}\xspace}
\newcommand{\mlist}{\ensuremath{\mathit{mlist}}\xspace}
%\newcommand{\Prob}{\ensuremath{\mathrm{P}}\xspace}
\newcommand{\eP}{\ensuremath{e_{\mathit{p}}}\xspace}
%\newcommand{\PLM}{\ensuremath{\Prob_{\mathrm{lm}}}\xspace}
% \newcommand{\PT}{\ensuremath{\Prob}\xspace}
% \newcommand{\PLex}{\ensuremath{\Prob_{\mathrm{lex}}}\xspace}

%NOW MOVED HERE
\newcommand{\npshift}{\hspace{1.6cm}}
\newcommand{\styleb}{linestyle=dashed}

\newcommand{\et}{\ensuremath{e^{\mathrm{t}}}}
\newcommand{\Ht}{\ensuremath{H^{\mathrm{t}}}}
%\newcommand{\ep}{\ensuremath{e^{\mathrm{p}}}}
\newcommand{\ep}{\ensuremath{e}\xspace}  % just for EMNLP
\newcommand{\Hp}{\ensuremath{H^{\mathrm{p}}}}
\newcommand{\Vp}{\ensuremath{V^{\mathrm{p}}}}

%\newcommand\newcite{\citet}
\def\namecite{\newcite}
%\def\namecite{\cite}

\def\Fone{F$_1$\xspace}
\def\Foneperc{F$_1\%$}
\newcommand{\goto}{\ensuremath{\triangleright}\xspace}

\newcommand{\TODO}[1]{\textbf{TODO:} \textit{#1}\xspace}

\newcommand{\smallnt}[1]{\ensuremath{_{\mbox{\tiny PP}}}\xspace}

\newcommand{\shift}{\ensuremath{\mathsf{sh}}\xspace}
\newcommand{\reduce}{\ensuremath{\mathsf{re}}\xspace}
\newcommand{\lreduce}{\ensuremath{\mathsf{re_{\small \curvearrowleft}}}\xspace}
\newcommand{\rreduce}{\ensuremath{\mathsf{re_{\small \curvearrowright}}}\xspace}


\newcommand{\sep}{\ensuremath{ \circ }\xspace}

\newcommand{\sttop}{\ensuremath{s_0}\xspace}
\newcommand{\stnext}{\ensuremath{s_1}\xspace}
\newcommand{\stthird}{\ensuremath{s_2}\xspace}
\newcommand{\qhead}{\ensuremath{q_0}\xspace}
\newcommand{\qnext}{\ensuremath{q_1}\xspace}
\newcommand{\qthird}{\ensuremath{q_2}\xspace}
\newcommand{\Tag}[1]{\ensuremath{{#1}.\mathsf{t}}\xspace}
\newcommand{\Wrd}[1]{\ensuremath{{#1}.\mathsf{w}}\xspace}
\newcommand{\LC}[1]{\ensuremath{{#1}.\mathsf{lc}}\xspace}
\newcommand{\RC}[1]{\ensuremath{{#1}.\mathsf{rc}}\xspace}

% Algorithm 3 -> Pseudocode 3
\newcommand{\pseudocode}{Algorithm}
\floatname{algorithm}{\pseudocode}

\newcommand{\cont}[2]{\ensuremath{\mathit{c}({#1}, {#2})}\xspace}
\newcommand{\contR}[2]{\ensuremath{\mathit{c}_{\mbox{\tiny \sc R}}({#1}, {#2})}\xspace}
\newcommand{\contsttops}{\ensuremath{\cont{\stnext}{\sttop}}\xspace}
\newcommand{\contsttopqhead}{\ensuremath{\contR{\sttop}{\qhead}}\xspace}

\newcommand{\sspan}{\ensuremath{\mathit{sp}}\xspace}
\renewcommand{\tspan}{\ensuremath{\mathit{tp}}\xspace}
\newcommand{\aspan}{\ensuremath{\mathit{ap}}\xspace}

% vanilla non-dp shift-reduce item: (l, S, Q)
\newcommand{\olditem}[3]{\ensuremath{{#1}: \tuple{{#2}, \ {#3}}}\xspace}
\newcommand{\newitem}[4]{\ensuremath{{#1}: \tuple{{#2}, \ {#3}, \ {#4}}}\xspace}

\newcommand{\arcs}{\ensuremath{\mathbf{a}}\xspace}
\newcommand{\arcleft}[2]{\ensuremath{{#1}^\curvearrowleft{#2}}\xspace}
\newcommand{\arcright}[2]{\ensuremath{{#1}^\curvearrowright{#2}}\xspace}

% kernel feature function
\newcommand{\vecfker}{\ensuremath{\widetilde{\mathbf{f}}}\xspace}
\newcommand{\fker}[1]{\ensuremath{\vecfker({#1})}\xspace}
\newcommand{\earleyitem}[3]{\ensuremath{\tuple{{#1}, {#2}, \ {#3}}}\xspace}
\newcommand{\nodpearleyitem}[2]{\ensuremath{\tuple{{#1}, \ {#2}}}\xspace}

\iffalse
\newcommand{\eisneritem}[4]{\newitem{#1}{#2}{#3}{\!\!\!\raisebox{0.04in}{\Tree[.{\ensuremath{#4}} !\Troof{\ensuremath{{#2}...{#3}}} ]}}\xspace}
\newcommand{\specialeisneritem}[4]{\newitem{#1}{#2}{#3}{#4}\xspace}
\else
\newcommand{\eisneritem}[4]{\tuple{{#1}, {\!\!\!\raisebox{0.04in}{\Tree[.{\ensuremath{#4}} !\Troof{\ensuremath{{#2}...{#3}}} ]}}\!\!\!}\xspace}
\newcommand{\specialeisneritem}[4]{\ensuremath{{#1}: \tuple{{#4}}}\xspace}
\newcommand{\gpeisneritem}[5]{\ensuremath{{#1}:\tuple{{#4}, {\!\!\!\raisebox{0.04in}{\Tree[.{\ensuremath{#5}} !\Troof{\ensuremath{{#2}...{#3}}} ]}}\!\!\!}}\xspace}
\fi

\newcommand{\decode}{\ensuremath{\mathit{decode}}\xspace}
\newcommand{\GEN}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\GENbar}{\ensuremath{\overline{\GEN}}\xspace}

\newcommand{\spb}[1]{\ensuremath{^{{#1}}}\xspace}
\newcommand{\spbkp}{\ensuremath{\spb{k+1}}\xspace}
\newcommand{\vecwk}{\ensuremath{\vecw\spb{k}}\xspace}
\newcommand{\vecwkp}{\ensuremath{\vecw\spb{k+1}}\xspace}
\newcommand{\vecwt}{\ensuremath{\vecw\spb{t}}\xspace}
\newcommand{\vecwtp}{\ensuremath{\vecw\spb{t+1}}\xspace}
\newcommand{\tth}{\ensuremath{t^{\mathrm{th}}}\xspace}


\newcommand{\err}{\ensuremath{\mathit{err}}\xspace}
\newcommand{\bPhi}{\ensuremath{\mathbf{\Phi}}\xspace}
\newcommand{\dPhi}{\ensuremath{\Delta\bPhi}\xspace}
\newcommand{\labels}{\ensuremath{\mathit{labels}}\xspace}
\newcommand{\onestep}{\ensuremath{\mathit{onestep}}\xspace}
\newcommand{\seqx}{\ensuremath{\overline{x}}\xspace}
\newcommand{\seqy}{\ensuremath{\overline{y}}\xspace}
\newcommand{\seqz}{\ensuremath{\overline{z}}\xspace}

\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\card}[1]{\lvert#1\rvert}  % cardinality |x|
\newcommand{\normtwo}[1]{\norm{#1}^2}

\newcommand{\seqzt}{\ensuremath{\overline{z}^{(t)}}\xspace}
\newcommand{\seqxt}{\ensuremath{\overline{x}^{(t)}}\xspace}
\newcommand{\seqyt}{\ensuremath{\overline{y}^{(t)}}\xspace}

\newcommand{\defeq}{\ensuremath{\stackrel{\Delta}{=}}\xspace}
\newcommand{\InlineIf}[2]{{\bf if} {#1} {\bf then} {#2}}
\newcommand{\dsep}{\ensuremath{\mathcal{D}(\vecu,\delta)}\xspace}
\newcommand{\dgsep}{\ensuremath{\mathcal{D}_g(\vecu,\delta)}\xspace}

\newcommand{\hinge}{\ensuremath{h_{\delta}}\xspace}

\newcommand{\Beam}{\ensuremath{\mathcal{B}}\xspace}

% equivalence class under ~: [[x]]_~
\newcommand{\eqvcls}[1]{\ensuremath{\llbracket {#1} \rrbracket_{\equiv}}\xspace}

\newcommand{\Cs}{\ensuremath{C_{\mathrm{s}}}}
\newcommand{\Cg}{\ensuremath{C_{\mathrm{g}}}}
\newcommand{\Cb}{\ensuremath{C_{\mathrm{b}}}}

%\newcommand{\state}{\ensuremath{\mathit{state}}\xspace}
\newcommand{\action}{\ensuremath{\mathit{action}}\xspace}


\newcommand{\fkerdp}[1]{\ensuremath{\vecfker_{{\mathrm{DP}}}({#1})}\xspace}
\newcommand{\fkernodp}[1]{\ensuremath{\vecfker_{\mathrm{noDP}}({#1})}\xspace}

\newcommand{\score}{\ensuremath{\mathit{S}}\xspace}
\newcommand{\scoring}[2]{\ensuremath{\score_{#1}({#2})}\xspace}
\newcommand{\scoresh}[1]{\ensuremath{\scoring{\shift}{#1}}\xspace}
\newcommand{\scoreleft}[1]{\ensuremath{\scoring{\lreduce}{#1}}\xspace}
\newcommand{\scoreright}[1]{\ensuremath{\scoring{\rreduce}{#1}}\xspace}

\newcommand{\leftptrs}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\rightptrs}{\ensuremath{\mathcal{R}}\xspace}

\newcommand{\chart}{\ensuremath{\mathit{C}}\xspace}
\newcommand{\pq}{\ensuremath{\mathit{Q}}\xspace}

\newcommand{\bleu}{{\sc Bleu}\xspace}
\newcommand{\bleuplusone}{\ensuremath{\mathrm{Bleu}^{+1}}\xspace}
\newcommand{\mert}{{\sc Mert}\xspace}
\newcommand{\ce}{{\sc Ch-En}\xspace}
\newcommand{\se}{{\sc Sp-En}\xspace}
\newcommand{\pro}{{\sc Pro}\xspace}
\newcommand{\mira}{{\sc Mira}\xspace}
\newcommand{\hols}{{\sc Hols}\xspace}
\newcommand{\ramp}{{\sc Ramp}\xspace}
\newcommand{\hiero}{{\sc Hiero}\xspace}
\newcommand{\cdec}{{\tt cdec}\xspace}

\newcommand{\MaxForce}{{\sc MaxForce}\xspace}

\newcommand{\myinfer}[3]{\ensuremath{\infer[\mbox{\footnotesize ${#1}$}]{#2}{#3}}\xspace}
\newcommand{\pre}{\ensuremath{\mathit{pre}}\xspace}
\newcommand{\good}{\ensuremath{\mathit{good}}\xspace}
\newcommand{\bad}{\ensuremath{\mathit{bad}}\xspace}
\newcommand{\ygood}{\ensuremath{\mbox{$y$-good}}\xspace}
\newcommand{\ybad}{\ensuremath{\mbox{$y$-bad}}\xspace}

\newcommand{\cn}{\ensuremath{{\sf cn}}\xspace}
\newcommand{\en}{\ensuremath{{\sf en}}\xspace}

\newcommand{\kNN}{\ensuremath{\mbox{$k$-NN}}\xspace}

\newcommand{\Yahoo}{{\sc Yahoo}\xspace}
\newcommand{\TREC}{{\sc TREC}\xspace}
\newcommand{\DMV}{{\sc DMV}\xspace}
\newcommand{\Insurance}{{\sc Insurance}\xspace}


\def\lr{\mbox{\begin{picture}(7,10)
\put(1,0){\line(1,0){5}}
\put(1,0){\line(1,2){5}}
\put(6,0){\line(0,1){10}}
\end{picture}
}}

%\def\ll{\mbox{\begin{picture}(7,10)
%\put(1,0){\line(1,0){5}}
%\put(6,0){\line(-1,2){5}}
%\put(1,0){\line(0,1){10}}
%\end{picture}
%}}

\def\llbig{\mbox{\begin{picture}(25,10)
\put(1,0){\line(1,0){30}}
\put(31,0){\line(-3,1){30}}
\put(1,0){\line(0,1){10}}
\end{picture}
}}

\def\lrbig{\mbox{\begin{picture}(25,10)
\put(1,0){\line(1,0){30}}
\put(1,0){\line(3,1){30}}
\put(31,0){\line(0,1){10}}
\end{picture}
}}
\newcommand{\doubleitem}[2]{\ensuremath{\stackrel{\!\!\!\!\!{#1}}{\ll} \stackrel{\ {#2}}{\lr}}\xspace}

\newcommand{\doubleitemleft}[2]{\ensuremath{\stackrel{\hspace{-0.9cm}{#1}}{\llbig} \quad \stackrel{\ {#2}}{\lr}}\xspace}


\newcommand{\doubleitemright}[2]{\ensuremath{\stackrel{\!\!\!\!\!{#1}}{\ll} \; \stackrel{\hspace{1.1cm} {#2}}{\lrbig}}\xspace}

\newcommand{\pytorch}{PyTorch\xspace}
\newcommand{\rnnsearch}{RNNsearch\xspace}

\newcommand{\best}{\ensuremath{\mathit{best}}\xspace}
\newcommand{\bestuptoi}{\ensuremath{\mathit{best}_{\leq i}}\xspace}
\newcommand{\completed}{\ensuremath{\mathit{comp}}\xspace}
\newcommand{\eos}{\mbox{\scriptsize \texttt{<eos>}}\xspace}
\newcommand{\bp}{\ensuremath{\mathit{bp}}\xspace}
\newcommand{\BLEU}{\ensuremath{\mathrm{BLEU}}\xspace}
\newcommand{\PWR}{\ensuremath{\mathrm{PWR}}\xspace}
\newcommand{\AdaR}{\ensuremath{\mathrm{AdaR}}\xspace}
\newcommand{\gnmt}{\ensuremath{\mathrm{GNMT}}\xspace}
\newcommand{\lengthnorm}{\ensuremath{\mathrm{length\_norm}}\xspace}
\newcommand{\word}{\ensuremath{\mathrm{word}}\xspace}
\newcommand{\len}{\ensuremath{\mathit{len}}\xspace}
\newcommand{\gratio}{\ensuremath{\mathit{gr}}\xspace}
\newcommand{\lratio}{\ensuremath{\mathit{lr}}\xspace}
\newcommand{\pred}{\ensuremath{\mathit{pred}}\xspace}

\newcommand{\spinyin}[1]{{\small\em {#1}}}
\newcommand{\bajisitan}{B\=aj\={\i}s\={\i}t\v{a}n}
\newcommand{\yindu}{Y\`{\i}nd\`u}

\newcommand{\deen}{{{de}$\leftrightarrow${en}}\xspace}
\newcommand{\zhen}{{{zh}$\leftrightarrow${en}}\xspace}
\newcommand{\detoen}{{{de}$\goesto${en}}\xspace}
\newcommand{\entode}{{{en}$\goesto${de}}\xspace}
\newcommand{\zhtoen}{{{zh}$\goesto${en}}\xspace}
\newcommand{\entozh}{{{en}$\goesto${zh}}\xspace}

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\gwaitk}{\ensuremath{{g_\text{wait-$k$}}}\xspace}
\newcommand{\gcatchup}{\ensuremath{{g_\text{wait-$k$, $c$}}}\xspace}

\newcommand{\waitk}{\ensuremath{\text{wait-$k$}}\xspace}

\newcommand{\CW}{\ensuremath{\mathrm{CW}}\xspace}
\newcommand{\AP}{\ensuremath{\mathrm{AP}}\xspace}
\newcommand{\AL}{\ensuremath{\mathrm{AL}}\xspace}


==> test.tex <==

Simultaneous translation has many important application scenarios and attracts many attentions in both academic and industry recently. Most existing frameworks, however, have difficulties in balancing between the translation quality and latency, i.e., the decoding policy usually is either too aggressive or too conservative. We propose an opportunistic decoding technique with timely correction ability, which always generates a certain mount of extra words at each step to keep the audience on track with the latest information, and in the meanwhile, our model also timely  corrects the former extra outputs with more observed context to ensure the translation quality. Experiments show our technique improves both latency and quality: an up to 2.4 RAL reduction and 3.1 BLEU improvement with revision rate under 8% in Chinese-to-English and English-to-Chinese (in appendix) translation. 
